LongForm: Effective Instruction Tuning with Reverse Instructions

Instruction tuning enables language models to more effectively generalize and better follow user intent. However, obtaining instruction data is costly and challenging. Prior work employs methods such as expensive human annotation, crowd-sourced datasets with alignment issues, and generating noisy examples via LLMs. We introduce the LongForm-C dataset, which is created by reverse instructions. We generate instructions via LLMs for human-written corpus examples using reverse instructions. First we select a diverse set of human-written documents from corpora such as C4 and Wikipedia; then we generate instructions for these documents via LLMs. This approach provides a cheaper and cleaner instruction-tuning dataset with natural output and one suitable for long text generation. Our models outperform 10x larger language models without instruction tuning on tasks such as story/recipe generation and long-form question answering. Moreover, LongForm models outperform prior instruction-tuned models such as FLAN-T5 and Alpaca by a large margin, and improve language understanding capabilities further. We publicly release our data and models: https://github.com/akoksal/LongForm.

==> table2.tex <==
	\begin{table*}[t]
		\footnotesize
		\setlength\tabcolsep{4.6pt}
		\centering
		\begin{tabular}{lrrrrrrrrrr}
			\toprule
			& \textbf{Model Size} &   \textbf{Avg.} & \textbf{C4} &  \textbf{Wiki} &  \textbf{SE} &  \textbf{HowTo} & \textbf{Enron} &  \textbf{BEA-GEC} &  \textbf{NIv2} &  \textbf{BigBench} \\
			
			\midrule
			T0++   & 11B  &   5.9 &   2.8 &   8.1 &    2.3 &    2.8 &    4.3 &     17.1 &                  11.3 &       1.7 \\
			T\textit{k}-Instruct  & 11B  &   6.0 &   2.2 &   9.4 &    3.2 &    1.3 &    3.8 &     12.4 &                  13.5 &       2.5 \\
			Flan-T5 &  11B & 12.5 &   4.1 &  13.3 &    5.8 &    4.1 &    8.4 &     70.8 &                  17.2 &       3.2 \\
			Alpaca-LLaMA-7B & 7B & 15.2 &   8.4 &  22.2 &    9.2 &   10.7 &    6.4 &     55.3 &                  16.9 &       8.6 \\
			\midrule
			OPT-30B & 30B  &  12.3 &  14.2 &  13.7 &   14.4 &    8.0 &    7.0 &     16.8 &                   9.5 &       3.3 \\
			\midrule
			\ModelName-T5-XL & 3B  &  24.3 &  18.9 &  22.4 &   15.3 &   21.5 &    8.7 &     \textbf{92.9} &                  \textbf{22.2} &      17.8 \\
			\ModelName-OPT-6.7B & 6.7B  &  24.2 &  \textbf{19.7} &  25.0 &   15.9 &   22.0 &    \textbf{8.9} &     85.1 &                  20.8 &      15.8 \\
			\ModelName-LLaMA-7B & 7B & \textbf{24.8} &  19.6 &  \textbf{27.8} &   \textbf{16.3} &   \textbf{22.6} &    6.6 &     86.2 &                  21.2 &      \textbf{18.0} \\
			\bottomrule
		\end{tabular}
		\caption{METEOR scores of baselines and our
			LMs on each subset 
			of \DataName
and micro
			average (``Avg.'') of the test set. All \ModelName models
			outperform prior LMs on long text
			generation with a big
			margin. \ModelName-T5-XL provides
			comparable results on text
			generation (i.e., tasks derived from BEA-GEC, NIv2 and BigBench), but the best results are achieved with \ModelName-LLaMA-7B.}
		\label{tab:res_writinginstructions}
	\end{table*}

